Eliciting Knowledge from Experts:Automatic Transcript Parsing for Cognitive Task Analysis

Cognitive task analysis (CTA) is a type of analysis in applied psychology aimed at eliciting and representing the knowledge and thought processes of domain experts. In CTA, often heavy human labor is involved to parse the interview transcript into structured knowledge (e.g., flowchart for different actions). To reduce human efforts and scale the process, automated CTA transcript parsing is desirable. However, this task has unique challenges as (1) it requires the understanding of long-range context information in conversational text; and (2) the amount of labeled data is limited and indirect---i.e., context-aware, noisy, and low-resource. In this paper, we propose a weakly-supervised information extraction framework for automated CTA transcript parsing. We partition the parsing process into a sequence labeling task and a text span-pair relation extraction task, with distant supervision from human-curated protocol files. To model long-range context information for extracting sentence relations, neighbor sentences are involved as a part of input. Different types of models for capturing context dependency are then applied. We manually annotate real-world CTA transcripts to facilitate the evaluation of the parsing tasks

==> previous_versions/feb22_1_introduction.tex <==
Cognitive task analysis (CTA) is a task in applied psychology to yield information about the knowledge and thought processes that underlie observable task performance of experts \cite{schraagen2000cognitive}. It is a powerful technique for training, instructional design \cite{clark1996cognitive, seamster2017applied}, and development of expert systems \cite{woods1989cognitive}. The traditional CTA methods require human-human interview, and involve human labor to analyze the interview record, to acquire the cognitive model, an approximation to human cognitive processes in structurized text, which is time consuming and requires domain experts. .

Recent years, techniques surged from the development of computer science are introduced to aid capturing human expertise \cite{Zhong:2015,etcta}. \citeauthor{li2013general}\shortcite{li2013general} used learning agent to discover cognitive model in specific domains. \citeauthor{cmwithnn}\shortcite{cmwithnn} explored modeling cognitive knowledge in well-setting tasks with neural models. However, for the most general setting that extracting cognitive processes from human-human interview, the heavy manual labor requirement to analyze interview transcript is still remained.

In this paper, we pursuit an automatic approach to extract cognitive processes from CTA interview transcript. Recent advances in machine reading comprehension, textual entailment \cite{bert} and relation extraction \cite{cotype, zhang2017position} shows the nowadays' NLP models earned the capability of capturing causual relation in some degree. Still, it is a open problem to extract procedural information from text. Some attempts to extract such information from well-structured instructional text are conducted by the information retrieval community \cite{codifyhowto} using OpenIE and hierarchical LSTM. However, our task is even more challenging since the CTA interview transcript we focusing on are unstructured conversational text, and the OpenIE technique applied by the previous studies cannot extract meaningful result.

!TODO! example of interview transcript, image openie result, protocol files

To address this problem, we introduce the manually analyzed cognitive models from CTA interview transcripts as protocols in a distant supervision manner. The protocols are well structured and summarizing cognitive processes mentioned in CTA interview. We 1) map the phrases in protocols back to the transcripts using fuzzy sentence matching techniques !TODO! section x; 2) use relation classification models on sentences in the transcripts with the supervision of structure information in protocols !TODO! section y; 3) to reduce literal expression gap between interview transcripts and summarized protocols, use sequence tagging models \cite{lmlstmcrf} to obtain summarized protocol phrases from sentences in transcripts !TODO! section z. With the approach above, we acquire the summarized sentences with structure relations and finally pack them into a cognitive model for CTA.

We evaluate our experiments from different extents: 1) evaluate the performance of different relation classification models and sequence labeling models with the same fuzzy sentence matching method !TODO! section a; 2) evaluate the performance of different fuzzy matching methods with the same relation classification model and sequence labeling model !TODO! section b; 3) evaluate the models and matching methods above independently with manually labeled data !TODO! section c. Our evaluation shows the effective of the approach.
